Humans as Path-Finders for Safe Navigation

One of the most important barriers toward a widespread use of mobile robots in unstructured and human populated work environments is the ability to plan a safe path. In this paper, we propose to delegate this activity to a human operator that walks in front of the robot marking with her/his footsteps the path to be followed. The implementation of this approach requires a high degree of robustness in locating the specific person to be followed (the leader). We propose a three phase approach to fulfil this goal: 1. identification and tracking of the person in the image space, 2. sensor fusion between camera data and laser sensors, 3. point interpolation with continuous curvature curves. The approach is described in the paper and extensively validated with experimental results.

==> Makefile <==
# Makefile for LaTeX files

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MAKETOC = "^[^%]*\\tableofcontents"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

PDFPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)
DEP	= *.tex

TRG	= $(SRC:%.tex=%.pdf)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false


all 	: $(TRG)

define run-latex
	  $(COPY);$(LATEX) $<
	  egrep -q $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(MAKETOC) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	  $(RM) $(<:%.tex=%.toc.bak)
	  # Display relevant warnings
	  egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

$(TRG)	: %.pdf : %.tex $(DEP) $(PDFPICS) $(BIBFILE)
	  @$(run-latex)

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.bbl) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)

.PHONY	: all show clean ps pdf showps

view:
	acroread $(PDF)

osx:
	open $(PDF)

######################################################################
# Define rules for PDF source files.
%.pdf: %.eps
	epstopdf $< > $(<:%.eps=%.pdf)

